Localization Uncertainty in Time-Amplitude Stereophonic Reproduction

This article studies the effects of inter-channel time and level differences in stereophonic reproduction on perceived localization uncertainty, which is defined as how difficult it is for a listener to tell where a sound source is located. Towards this end, a computational model of localization uncertainty is proposed first. The model calculates inter-aural time and level difference cues, and compares them to those associated to free-field point-like sources. The comparison is carried out using a particular distance functional that replicates the increased uncertainty observed experimentally with inconsistent inter-aural time and level difference cues. The model is validated by formal listening tests, achieving a Pearson correlation of 0.99. The model is then used to predict localization uncertainty for stereophonic setups and a listener in central and off-central positions. Results show that amplitude methods achieve a slightly lower localization uncertainty for a listener positioned exactly in the center of the sweet spot. As soon as the listener moves away from that position, the situation reverses, with time-amplitude methods achieving a lower localization uncertainty.

==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------

\usetikzlibrary{arrows, calc, positioning, decorations.markings}

% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\tikzset{
	buffer/.style={
		draw,
		shape border rotate=180,
		regular polygon,
		regular polygon sides=3,
		fill=red,
		node distance=2cm,
		minimum height=4em
	}
}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclaretriangleoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
		\saveddimen\radius
		{
			\pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
			\pgfmathsetlength\pgf@ya{\pgfshapeminheight}
			\ifdim\pgf@xa>\pgf@ya
			\pgf@x=.5\pgf@xa
			\else
			\pgf@x=.5\pgf@ya
			\fi
		}
		
		% Inherit all anchors from the 'circle'-shape:
		\inheritanchor[from={circle}]{center}
		\inheritanchor[from={circle}]{mid}
		\inheritanchor[from={circle}]{base}
		\inheritanchor[from={circle}]{north}
		\inheritanchor[from={circle}]{south}
		\inheritanchor[from={circle}]{west}
		\inheritanchor[from={circle}]{east}
		\inheritanchor[from={circle}]{mid west}
		\inheritanchor[from={circle}]{mid east}
		\inheritanchor[from={circle}]{base west}
		\inheritanchor[from={circle}]{base east}
		\inheritanchor[from={circle}]{north west}
		\inheritanchor[from={circle}]{south west}
		\inheritanchor[from={circle}]{north east}
		\inheritanchor[from={circle}]{south east}
		\inheritanchorborder[from={circle}]
		
		% Draw circle and embed additional code
		\backgroundpath
		{
			% Draw circle
			%\pgfpathpolygon{\centerpoint}{\pgfpoint{1em}{1em}}
			 \pgfpathmoveto{\centerpoint} 
			 \pgfpathmoveto{\pgfpoint{0cm}{-\radius}} 
			\pgfpathlineto{\pgfpoint{\radius}{\radius}} 
			\pgfpathlineto{\pgfpoint{-\radius}{\radius}} 
			\pgfpathlineto{\pgfpoint{0}{-\radius}} 
			
			% Embed additional code
			% (Note that this code must call e.g. \pgfusepathqstroke
			#2
		}
		
		% Define anchor parametrized by the PGF key /tikz/dsp/label
		\anchor{text}
		{
			\centerpoint
			%
			\def\templabelabove{above}
			\def\templabelbelow{below}
			\def\templabelleft{left}
			\def\templabelright{right}
			\pgfutil@tempdima=\dspoperatorlabelspacing
			%
			\ifx\label\templabelabove
			\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
			\advance\pgf@y by \radius
			\advance\pgf@y by \pgfutil@tempdima
			\fi
			%
			\ifx\label\templabelbelow
			\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
			\advance\pgf@y by -\radius
			\advance\pgf@y by -\pgfutil@tempdima
			\advance\pgf@y by -\ht\pgfnodeparttextbox
			\fi
			%
			\ifx\label\templabelleft
			\advance\pgf@x by -\radius
			\advance\pgf@x by -\pgfutil@tempdima
			\advance\pgf@x by -\wd\pgfnodeparttextbox
			\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
			\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
			\fi
			%
			\ifx\label\templabelright
			\advance\pgf@x by \radius
			\advance\pgf@x by \pgfutil@tempdima
			\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
			\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
			\fi
		}
	}
}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclaretrianglehorzoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
		\saveddimen\radius
		{
			\pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
			\pgfmathsetlength\pgf@ya{\pgfshapeminheight}
			\ifdim\pgf@xa>\pgf@ya
			\pgf@x=.5\pgf@xa
			\else
			\pgf@x=.5\pgf@ya
			\fi
		}
		
		% Inherit all anchors from the 'circle'-shape:
		\inheritanchor[from={circle}]{center}
		\inheritanchor[from={circle}]{mid}
		\inheritanchor[from={circle}]{base}
		\inheritanchor[from={circle}]{north}
		\inheritanchor[from={circle}]{south}
		\inheritanchor[from={circle}]{west}
		\inheritanchor[from={circle}]{east}
		\inheritanchor[from={circle}]{mid west}
		\inheritanchor[from={circle}]{mid east}
		\inheritanchor[from={circle}]{base west}
		\inheritanchor[from={circle}]{base east}
		\inheritanchor[from={circle}]{north west}
		\inheritanchor[from={circle}]{south west}
		\inheritanchor[from={circle}]{north east}
		\inheritanchor[from={circle}]{south east}
		\inheritanchorborder[from={circle}]
		
		% Draw circle and embed additional code
		\backgroundpath
		{
			% Draw circle
			%\pgfpathpolygon{\centerpoint}{\pgfpoint{1em}{1em}}
			\pgfpathmoveto{\centerpoint} 
			\pgfpathmoveto{\pgfpoint{-\radius}{\radius}} 
			\pgfpathlineto{\pgfpoint{\radius}{0}} 
			\pgfpathlineto{\pgfpoint{-\radius}{-\radius}} 
			\pgfpathlineto{\pgfpoint{-\radius}{\radius}} 
			
			% Embed additional code
			% (Note that this code must call e.g. \pgfusepathqstroke
			#2
		}
		
		% Define anchor parametrized by the PGF key /tikz/dsp/label
		\anchor{text}
		{
			\centerpoint
			%
			\def\templabelabove{above}
			\def\templabelbelow{below}
			\def\templabelleft{left}
			\def\templabelright{right}
			\pgfutil@tempdima=\dspoperatorlabelspacing
			%
			\ifx\label\templabelabove
			\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
			\advance\pgf@y by \radius
			\advance\pgf@y by \pgfutil@tempdima
			\fi
			%
			\ifx\label\templabelbelow
			\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
			\advance\pgf@y by -\radius
			\advance\pgf@y by -\pgfutil@tempdima
			\advance\pgf@y by -\ht\pgfnodeparttextbox
			\fi
			%
			\ifx\label\templabelleft
			\advance\pgf@x by -\radius
			\advance\pgf@x by -\pgfutil@tempdima
			\advance\pgf@x by -\wd\pgfnodeparttextbox
			\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
			\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
			\fi
			%
			\ifx\label\templabelright
			\advance\pgf@x by \radius
			\advance\pgf@x by \pgfutil@tempdima
			\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
			\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
			\fi
		}
	}
}


\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclaretriangleoperator{dspshapemultiplier}{

\pgfusepathqstroke
}

\dspdeclaretrianglehorzoperator{dspshapemultiplierhorz}{
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother

% -------------------------------------------------------------------------
% Define node styles

\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspmultiplierhorz/.style={shape=dspshapemultiplierhorz,line cap=rect,line join=rect,
		line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
	
\tikzset{dspmultiplier/.style={shape=dspshapemultiplier,line cap=rect,line join=rect,
		line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}

% -------------------------------------------------------------------------
% Define "signal flow" lines

\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

